Resilient Edge: Can we achieve Network Resiliency at the IoT Edge using LPWAN and WiFi?

Edge computing has gained attention in recent years due to the adoption of many Internet of Things (IoT) applications in domestic, industrial and wild settings. The resiliency and reliability requirements of these applications vary from non-critical (best delivery efforts) to safety-critical with time-bounded guarantees. The network connectivity of IoT edge devices remains the central critical component that needs to meet the time-bounded Quality of Service (QoS) and fault-tolerance guarantees of the applications. Therefore, in this work, we systematically investigate how to meet IoT applications mixed-criticality QoS requirements in multi-communication networks. We (i) present the network resiliency requirements of IoT applications by defining a system model (ii) analyse and evaluate the bandwidth, latency, throughput, maximum packet size of many state-of-the-art LPWAN technologies, such as Sigfox, LoRa, and LTE (CAT-M1/NB-IoT) and Wi-Fi, (iii) implement and evaluate an adaptive system Resilient Edge and Criticality-Aware Best Fit (CABF) resource allocation algorithm to meet the application resiliency requirements using Raspberry Pi 4 and Pycom FiPy development board having five multi-communication networks. We present our findings on how to achieve 100% of the best-effort high criticality level message delivery using multi-communication networks

==> Images/Exp/exp1.tex <==
\begin{figure}
\begin{tikzpicture}
  \begin{axis}[
    ybar,
    height = 5cm,  
	width=\columnwidth,    
    enlargelimits=0.15,
%    legend style={at={(0.5,-0.2)},anchor=north,legend columns=-1},
    ylabel={Time (ms)},
    symbolic x coords={FiPy,RPi,},
    xtick=data,
    xlabel near ticks,
    ylabel near ticks,
    nodes near coords, 
	nodes near coords align={vertical},
%    x tick label style={rotate=45,anchor=east},
    ]
    \addplot coordinates {(FiPy,1077)};
    \addplot coordinates {(RPi,7.1)};
    \legend{FiPy, RPI}
  \end{axis}
\end{tikzpicture}
\caption{Running time of an algorithm on RPI and FiPy board.}
\label{fig:exp-1}
\end{figure}

==> Images/Exp/exp2.tex <==
\begin{figure}
\begin{tikzpicture}
	\begin{axis}[%
	x label style={anchor=north},
    ylabel near ticks,
    xlabel near ticks,
    y label style={anchor=south},
    xlabel={$\%$ services message flows},
    ylabel={average allocated criticality level},
    xmax=1.1, xmin=0,
    ymax=3.1, ymin=0.9,
%    legend style={anchor=east west,legend columns=1},
    legend style={at={(0.02,0.02)},anchor=south west},
    legend entries={\wifi,\lora,\nbiot,\sigfox,WiFi+LoRa, WiFi+Sigfox, NB-IoT+LoRa, NB-IoT+Sigfox},    
	%clickable coords={(xy): \thisrow{label}},%
	scatter/classes={%
		WiFi={mark=square,black},%
		LoRa={mark=triangle,black},%
		NB-IoT={mark=asterisk,black},%
		Sigfox={mark=x,draw=black},	
		WiFiLoRa={mark=+,draw=black},
		WiFiSigfox={mark=o,draw=black},
		NB-IoTLoRa={mark=diamond,draw=black},
		NB-IoTSigfox={mark=pentagon,draw=black},
		H_WiFi={mark=square,red},%
		H_LoRa={mark=triangle,red},%
		H_NB-IoT={mark=asterisk,red},%
		H_Sigfox={mark=x,draw=red},	
		H_WiFiLoRa={mark=+,draw=red},
		H_WiFiSigfox={mark=o,draw=red},
		H_NB-IoTLoRa={mark=diamond,draw=red},
		H_NB-IoTSigfox={mark=pentagon,draw=red},		
		c={mark=o,draw=black}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x   y      label
1   1     WiFi 
1   1.625   Sigfox
1   1   NB-IoT
1   1   WiFiLoRa
1   1   WiFiSigfox
1  1.25 LoRa
1   1.75    H_WiFi
0.25   3  H_Sigfox
1   2   H_NB-IoT
0.75    2.33    H_LoRa
1   1.75    H_WiFiLoRa
1   1.75    H_WiFiSigfox
1   1.875   H_NB-IoTLoRa
1   2   H_NB-IoTSigfox
	};
	\end{axis}
\end{tikzpicture}
\label{fig:alloc_crit_percent}
\caption{Allocated criticality and percentage for different network scenarios for different payloads. The marker with black color represents the payload defined in \autoref{tab:AssistedLivingExample} and red color represents the payload with 100,000 times the payload at Criticality level 0 and 5000 times the payload at Criticality level 1.}
\end{figure}

==> Images/pin_out.tex <==
%\usepackage{tikz}
\usetikzlibrary{calc}           % For general calculations
\usetikzlibrary{matrix}         % For the matrix cmd
\usetikzlibrary{positioning}    % For above = Xcm of and similars
\usetikzlibrary{intersections}  % Mainly here for the arc over line
\usetikzlibrary{topaths}        % Enable move to operation

%%% Adapted from https://tex.stackexchange.com/a/111674/114143
%%% provides syntax for jumping lines
\tikzset{
    connect/.style args={(#1) to (#2) over #3 by #4}{
        insert path={
            \pgfextra{
                \pgfinterruptpath
                    \path [name path=userpath] (#1) -- (#2);
                    \path [name intersections={of=userpath and #3,by=overpoint}];
                \endpgfinterruptpath                
            }
            let \p1=($(#1)-(overpoint)$), \n1={veclen(\x1,\y1)}, 
                            \n2={atan2(\y1,\x1)}, \n3={abs(#4)}, \n4={#4>0 ?180:-180}  in 
                            (#1) -- ($(#1)!\n1-\n3!(overpoint)$) 
                            arc (\n2:\n2+\n4:\n3) -- (#2)
        }
    },
}

%% Block styles (to avoid repetition and ease our lives)
\tikzset{wire board/.style={matrix of nodes,
                            row sep=2mm,
                            nodes={anchor=center}
                            },
        lidar/.style={column 1/.style={nodes={left}},
                                       column 3/.style={nodes={above right}},
                                       column 2/.style={font=\bfseries}
                                       },
        rj542/.style={column 1/.style={nodes={above left}},
                                       column 3/.style={nodes={right}}
                                       },
        scpb/.style={rj542,
                     column 2/.style={font=\bfseries}
                     }
}

\sffamily
%\begin{figure}
\begin{tikzpicture}
%% Drawing the first block (LIDAR)
\matrix[wire board,lidar] (Lidar) {
        &   2    &   5V   \\
        &   4    &   5V   \\
        &   6    &   GND   \\
  TXD   &   8    &   GPIO14   \\
  RXD   &   10   &   GPIO15   \\
        &   12   &   GPIO18   \\
        &   14   &   GPIO18   \\
        &   16   &   GPIO18   \\
 %       &   18   &   GPIO18   \\
 %       &   20   &   GPIO18   \\
 %       &   22   &   GPIO18   \\        
 %       &   24   &   D-007   \\
 %       &   26   &   GPIO18   \\
 %       &   28   &   GPIO18   \\
 %       &   30   &   GPIO18   \\
 %       &   32   &   GPIO18   \\
 %       &   34   &   GPIO18   \\
 %       &   36   &   GPIO18   \\
 %       &   38   &   GPIO18   \\
 %       &   40   &   GPIO18   \\
};
% Boxing the contents
  \draw (Lidar-1-2.north east) rectangle (Lidar-8-2.south west);
  \draw (Lidar-1-2.north west)+(-5cm,0.5cm) node[above right, font=\bfseries]{Raspberry Pi} rectangle ($(Lidar-8-2.south west)+(0,-0.5cm)$);

%% Drawing the second block (RJ45)
\matrix[wire board, rj542, matrix anchor=north, right=9cm of Lidar.north] (RJ542) {
  RST &  9  &   \\
  P0 &   40   &   RX0 \\
  P1 &   41   &   TX0 \\
  P2 &   23   &       \\
  P3 &   24   &   TX1     \\
  P4 &   21   &   RX1 \\
  CLK &   34   &       \\
%  MOSI &   16   &       \\
%  MISO &   38   &       \\
%  P8 &   22   &       \\
%  P9 &   18   &       \\
%  P10 &   20   &       \\
%  P11 &   39   &       \\
%  P12 &   42   &       \\  
};
% Boxing the contents
  \draw (RJ542-1-2.north east) rectangle (RJ542-7-2.south west);
  \draw (RJ542-1-2.north east)+(0cm,0.5cm) node[above right, align=center]{Pycom FiPy} rectangle ($(RJ542-7-2.south east)+(5cm,-0.5cm)$);

%% Connecting the wires
%\draw (Lidar-3-2) -- +(2.00cm,0) |- (RJ542-8-2.200);
\draw (Lidar-4-2) -- +(5.25cm,0) |- (RJ542-6-2);
\draw (Lidar-5-2) -- +(3.00cm,0) |- (RJ542-5-2);
\end{tikzpicture}                       
%\end{figure}

==> Sections/Dump.tex <==
\subsubsection*{\textbf{Exp-02: Sending data with different network interfaces}}
For a device to have resiliency, it will need to send the data with all networks at the same time. To understand whether the FiPy device can send the data at all interfaces at the same time and if there are any bottlenecks or performance issues. We send a simple message "HelloWorld12" repeated of length 240 bytes continuously on Wi-Fi, LoraWAN using a while loop. In case of Wi-Fi and Sigfox, we were able to send the message without any sleep, however for Lora we used three seconds sleep with a try and catch block as we received OSError: [Errno 11] EAGAIN for Lora network. This error might occur as sending a LoRaWAN packet (as per-protocol specs) takes more than 1 second because the device needs to wait for the first receive window (which occurs 1 second after the packet is sent). We further performed the latency, bandwidth and throughput tests for WiFi. We did try to send messages at all interface Lora/Sigfox/Wi-Fi, however, we repetitively received OSError: [Errno 11]. This might be because Sigfox and Lora use the same antenna. When we were transferring data using Wi-Fi and Lora continuously, \autoref{fig:exp1_wifi_latency}, \autoref{fig:exp1_wifi_bandwidth}, \autoref{fig:exp1_wifi_throughput} provides latency, bandwidth and throughput of the Wi-Fi network when machine pinged, iperf server is stored locally in the same network and remotely in the cloud network. Latency has an average of 5.73 ms/ 14.84 ms with a standard deviation of 1.12 ms/ 1.12 ms for the machine in a local and remote network, respectively. Bandwidth has an average of 3231.1/ 733.64 Kbits/ sec with a standard deviation of 173.3909869/ 23.36 when iperf3 is hosted locally in the same network and cloud network.

\input{Images/exp1_wifi_bandwidth}
\input{Images/exp1_wifi_latency}
\input{Images/exp1_wifi_throughput}
\subsection{Previous Implementations?}
The array of Things? 

\subsection{Architecture}

A raspberry-Pi running docker instances for 
\begin{itemize}
    \item Video analytics either counting number of pedestrians, cars; counting number of people on the bus stops; ANPR; Face Recognition (By permission of law-enforcement under emergency circumstances); analyse whether people are maintaining social distance 2meter distance because of COVID-19. \notevk{ Check how feed can be saved locally or streamed for law enforcement agencies with security (if required). Multiple views of the data? How?}
    \item audio analytics understanding the environment for noise maps or classifying the sounds into different types such as sounds of birds, gunshots.
    \item Environment monitoring - Air Pollution
    \item Internet sharing at deprived areas? Allowing people to share their internet with control on what is allowed on the Wi-Fi? 
\end{itemize}

Raspberry Pi might be connected with FiPy\footnote{FiPy \url{https://pycom.io/product/fipy/}} which has multiple network connectivity options such as LTE, Wi-Fi, LoRa, SigFox, NB-IoT, Bluetooth. It would be interesting to explore multi-tenancy based on different network, sending different data over different network.

\notevk{ Look into - How bandwidth, QoS can be set on docker containers?}
\notevk{Look into Internet Sharing from RasberryPi/ Jetson Nano and how we can control the internet usage}
\notevk{How to implement Policies}


%\subsection{Python Implementation}
%\begin{enumerate}
    \item Define the message flow and application with criticality level, message size, frequency.
    \item Simulate the above message flows from the AppX
    \item Determine the bandwidth of the bins (network interfaces - Sigfox/ LoRa/ LTE/ WiFi)
    \item Create a network interface (function) for the bins to send the message with specified bandwidth.
    \item Assign the message flow with required bandwidth to specified network interface by determining how much bandwidth is left and set accordingly.
    \item From the above, we should have a matrix specifying message flow with C bytes and T frequency should be routed via network interface.
    \item Continuously check the network interfaces status (at-least for WiFi and LTE) and update the current state matrix (message flow -> network interface).
    \item When a particular application with particular message flow wants to send the message, it refers to the matrix (checks whats the message size and frequency it can send). If the message size is acceptable, it forwards it to the particular network bin, else reduce the message size (change itself to different critically level) and then send.
%\end{enumerate}

==> Sections/IoTDI_Review.tex <==
\subsection{Reviewer 1}
- The work targets at the QoS requirements of multi-communication networks where IoT devices are equipped with multiple network interfaces. It is unclear whether all network interfaces are powered on when the IoT devices are operating. If so, the power consumption will be a matter of concern. Otherwise, IoT devices need to switch between network interfaces and turning on/off interfaces. The overhead of switching would be a problem.
\notevk{Maybe, we can mention a note in Discussions section that "Currently, all the network interfaces are initialised at the boot. However, the connection to the network is based on network availability and conditions. For instance, if the Wi-Fi network is available, NB-IoT is not connected; if LoRa network is joined successfully, Sigfox socket is not created. Further, we have mentioned the connect times for different technologies (sec 5.1) time to connect to network, which can be considered as switching time? with context switching in sec 6.2? }

- When the authors manage multi-network resource to meet QoS requirements of IoT applications, they only determine which network interface (e.g., LoRa, SigFox or WiFi) should be used for transmitting a specific type of message. Yet the communication parameters of the selected technology is not determined. For example, how exactly a LoRa interface should be configured (e.g., spreading factor, channel) to transmit a message is not described. The formulated QoS allocation problem should also consider the communication parameters of different network interfaces.
\notevk{We do consider the communication parameters of different network interfaces. For instance, when a network interface is defined (whether it is available or not), we do define the bandwidth available (function define\_networks in boot script). In case of Lora, when lora starts connecting, the spreading factor is adaptive i.e it would start with SF7, if it can't connect with SF7, it would try with SF8 and so on. We take the bandwidth of the connected spreading factor }

- In Sec 4.1, when the authors formulate the QoS allocation problem as an Integer Linear Programming problem, they assumes that the QoS requirements of all applications can be satisfied. Yet, in practice, the network capability is limited. It is not known whether the method can handle the case that some applications’ QoS requirements cannot be satisfied by the network capability.
\notevk{Does the reviewer meant that there can be applications QoS which cannot be satisfied by any network? (for instance Wi-Fi can satisfy most of the QoS requirements?)}

- In Sec 4.2, it seems that the authors try to use some existing algorithms to solve their problem, which somehow limits the contribution of this paper. In addition, it would be better to clearly present how the required inputs of Algorithm 1 are provided? Are they collecting from the edge devices? or should they be provided by the app designers?
\notevk{We did mention application developers a few times (although not in sec 4.2). Maybe we can add "defined by application developers" after "Algorithm 1 describes the proposed CABF algorithm, which
takes as inputs the sets T of message flows" in sec 4.2?}

- Network dynamic is not considered. As the wireless channel and link conditions will change dynamically. How the proposed CABF algorithm handles network dynamic is not discussed in the paper. \notevk{LoRa and SigFox do not really have any connection status, as they are not continuously connected. Regarding Wi-Fi, pycom devices does not provide any callback functionality yet (we mentioned this in the discussion section). Regarding LTE, Pycom has implemented callback functionality in Nov 2020, the code can be implemented}

- Section 5.1 provide too much background information in terms of payload length, throughput, latency etc, most of which can be obtained from the datasheet of corresponding devices and are not very relevant to the evaluation work of this paper. It looks more like a background introduction.
\notevk{Ok, Will cut down}

\subsection{Reviewer 2}
\subsubsection{Strengths}

- A Resilient prototype has been implemented  and executed for two types of applications (HealthAppa nd HomeApp). So far, It has only taken  bandwidth and inter-message period  into account for defining  criticality.

\subsubsection{Weaknesses}

- Section 5.1  on evaluation metrics needs to be improved and should further  highlight the more important information to be retained. The section  is indeed presented as a catalog of metrics and of technologies. Some figures have also to be further commented: for example, Fig.4.
\notevk{Ok, Will cut down. Not sure what the reviewer meant by "further commented", Removed?}

- In the evaluation section, Section 6.2 could be more detailed. It would be interesting to generate some network problems during application communication and then to evaluate the consequences on the flows (latency, loss, throughput).
\notevk{Good idea. The problem is creating network problems is maybe a little difficult as of now. For instance, Regarding Wi-Fi, we can turn on/off the wifi connectivity, however pycom doesn't provide the callback function. For LTE, we can possibly remove the SIM card, while it is on? or remove the LTE antenna (although not recommended officially), Lora and Sigfox are stateless? Lora get joined, but no way to find whether it is still connected? Nevertheless we can write about these constrains specifically. }

\subsection{Reviewer 3}
\subsubsection{Pros}
The author claims that they have opened up a new research direction, which is correct to a certain extent. Resilient Edge can be considered as a study on how services on the IoT edge continue to work normally in the event of a network failure.     

This work helps build reliable applications on IoT Edge, and provides solutions from the perspective of communication networks to improve service quality and fault tolerance on resource-constrained edge devices.

The author has completed a systematic work, from the definition of the message flow, including the byte size, interval and level of the message, as well as the proposed maximization objective function and CABF algorithm, to implementation and evaluation. The author proposed a resource management algorithm-Criticality-Aware Best Fit (CABF) algorithm, and proposed two variants of the algorithm, which can achieve good results.

In the introduction, evaluation, and discussion sections, the author has made a detailed description of several different networks used, including their characteristics, differences and limitations.

The author conducted comparative experiments on multiple communication networks using different fitting algorithms, and the chart presentation and description logic are clear.

\subsubsection{Cons}
- The author did not explain how the data in Table 1 came from. These data are needed by the author's experiments and algorithms. Because they don't seem to be obtained through experiments, if the author set it intuitively, the author should give the basis or reason for such setting, so that users can easily extend the research of this article to their own applications.
\notevk{We missed mentioning this, I believe we set this intuitively? or maybe referred a dataset?}

- In section 4.1, the author said that more indicators can be considered for network resource management, and that this is easy but will be reserved for future work, and only considers bandwidth capacity and utilization. In the current work, the author can consider such things as the size of the maximum payload and the maximum number of messages per day, which may directly limit certain or certain types of network resources. For example, Sigfox only allows up to 140 messages per day. \notevk{Can work on this and implement size of maximum payload and max number of messages}

- With the development and popularization of 4G/5G networks, the IoT edge has also shown more possibilities. The Internet of Everything, VR, and AI intelligence may all be features that edge devices will have. In this context, "NB-IoT UL (55 Kbps), LoRa SF7-125KHz (5.47 Kbps) Sigfox UL (100 bps) these low-bandwidth network communication methods are very limited. I would like to see the author talk about the relationship between the most advanced technology of the network and their work. \notevk{Not sure, Should we mention something like "our work targets edge applications with limited bandwidth requirements? }

- Starting in Chapter 5.1, the author spent about three pages to describe the evaluation, but these contents do not read coherently with the previous content of Chapter 5.1. It seems that due to insufficient experimental results in the Resilient Edge design part, the author added these pages.
\notevk{Ok, Will cut down from section 5.1}

\subsection{Reviewer 4}
The paper is written in a fluent manner. The analysis of use-cases seems clear. The new criticality-aware QoS allocation problem based on VSBPP seems novel and rigorous. The ILP formulation method and Bin-Packing Algorithms seems robust. The experiments are done in a rigorous manner and the results seem ideal.  However, the paper still has some drawbacks listed as follows.

- The system model mentioned in section 3 seems not clear. The authors only demonstrated some basic characteristics of the model, without showing the detailed components as well as the flow of the model. The authors need to give some detailed explanation of the system model, probably with some flowcharts and graphs. \notevk{Can possibly create flow chart, not sure about the graph and more detailed components.}

- The authors mentioned that the new system is an adaptive system, which means that it is suitable for different types of applications. However, in Table 1, the author only mentioned Health Apps and Home Apps. Additionally, the explanation or demonstration of the new model`s adaptive ability under different environments seems not enough in the paper. The authors need to add further discussions or contents about this. \notevk{Maybe we want to specify that Health Apps and Home Apps are sample applications?}

- In the experiment part, the authors mentioned that prototypes of HealthApp and HomeApp are implemented and used. However, details of these two Apps like work flows or functions are not clear enough. Authors should provide more details of those Apps or attach the source code to reference.
\notevk{In section 5, Maybe, we should change the language from prototyped to simulated the message flow?}

- The experiment part seems a little bit insufficient since the author did not take the external factors, such as the intensity of Wi-Fi signals or surrounding environments into consideration. Further experiments need to be conducted under different external factors.
\notevk{Umm...External factors such as intensity of Wi-Fi signals/ surrounding environments? difficult to consider? Plus, no Wi-Fi callback}


==> Sections/acro.tex <==
\begin{acronym}
\acro{6LoWPAN}{IPv6 over Low Power Wireless Personal Area Networks}
\acro{RF}{Radio frequency}
\acro{RSSI}{Received Signal Strength Indicator}
\acro{LQI}{Link Quality Indicator }
\acro{SCK}{Smart Citizen Kit}
\acro{eCO2}{equivalent CO2}
\acro{UO}{Urban Observatory}
\acro{IoT}{Internet of Things}
\acro{WSN}{Wireless Sensor Networks}
\acro{SHM}{Structural Health Monitoring}
\acro{BSI}{British Standards Institute}
\acro{ICT}{Information and Communications Technology}
\acro{SolarPV}{Solar Photovoltaic Systems}
\acro{KPI}{Key Performance Indicators}
\acro{MCU}{Microcontrollers}
\acro{APNR}{Automatic Plate Number Recognition}
\acro{CCTV}{Closed-circuit television}
\acro{CO}{Carbon Monoxide}
\acro{CO2}{Carbon Dioxide}
\acro{NO}{Nitric Oxide}
\acro{NO2}{Nitrogen Dioxide}
\acro{CH4}{Methane}
\acro{H2S}{Hydrogen sulfide}
\acro{NH3}{Ammonia}
\acro{ECG}{Electrocardiogram}
\acro{LIDAR}{Light Detection and Ranging}
\acro{NOAA}{National Oceanic and Atmospheric Administration}
\acro{LTE}{Long Term Evolution}
\acro{GPRS}{General Packet Radio Service}
\acro{CDMA}{Code-division multiple access}
\acro{GSM}{Global System for Mobile Communication}
\acro{NB-IoT}{Narrowband IoT}
\acro{M2M}{Machine to Machine}
\acro{WiMAX}{Worldwide Interoperability for Microwave Access}
\acro{UWB}{Ultra Wideband}
\acro{BUO}{Bristol Urban Observatory}
\acro{LAN}{Local Area Network}
\acro{RFID}{Radio-frequency identification}
\acro{NFC}{Near-field communication}
\acro{BCG}{Ballistocardiographic}
\acro{PIR}{Passive Infrared Sensor}
\acro{IAQ}{Indoor Air Quality}
\acro{VOC}{Volatile Organic Compounds}
\acro{EV}{Electric Vehicle}
\acro{TfL}{Transport for London}
\acro{TERS}{Temporary earth restraining structure}
\acro{SLA}{Service level agreement}
\acro{LoRaWAN}{Long Range Wide Area Network}
\acro{WiMAX}{Worldwide Interoperability for Microwave Access}
\acro{MINA}{Multinetwork INformation Architecture}
\acro{AoT}{Array of Things}
\acro{OAA}{Observe Analyse Adapt}
\acro{SBC}{Single Board Computer}
\acro{SPHERE}{Sensor Platform for HEalthcare in a Residential Environment}
\acro{SHG}{SPHERE Home Gateway}
\acro{SDH}{SPHERE Data Hub}
\acro{NUC}{Next Unit of Computing}
\acro{LCD}{Liquid Crystal Display}
\acro{SONET}{Synchronous optical networking}
\acro{DSL}{Digital Subscriber Line}
\acro{LED}{Light Emitting Diode}
\acro{SoC}{System on Chip}
\acro{TBI}{Traumatic Brain Injury}
\acro{AURN}{Automatic Urban and Rural Network}
\acro{VOCS}{Volatile Organic Compounds}
\acro{QoL}{Quality of Life}
\acro{AQI}{Air Quality Index}
\acro{UKCRIC}{UK Collaboratorium for Research On Infrastructure and Cities}
\acro{NAK}{Network Authentication Key}
\acro{MAC}{Message Authentication Code}
\acro{APN}{Access Point Names}
\acro{DoNAS}{Data over NAS}
\acro{NIDD}{Non-IP Data Delivery}
\acro{SIM}{Subscriber Identity Modules}
\acro{UNB}{Ultra-Narrow Band}
\acro{ADR}{Adaptive Data Rate}
\acro{QoS}{Quality of Service}
\acro{PSM}{Power Saving Mode}
\acro{ILP}{Integer Linear Programming}
\acro{UE}{User Equipment}
\acro{TTN}{The Things Network}
\acro{eDRX}{Extended Discontinuous reception}
\acro{OTAA}{Over-the-air Activation}
\acro{ABP}{Activation-by-personalization}
\acro{MIC}{Message Integrity Code}
\acro{PLMN}{Public Land Mobile Network}
\acro{DL}{down-link}
\acro{UL}{up-link}
\acro{MTU}{Maximum Transmission Unit}
\acro{TCP}{Transmission Control Protocol}
\acro{IP}{Internet Protocol}
\acro{SF}{Spreading Factor}
\acro{WPA}{Wi-Fi Protected Access}
\acro{WPS}{Wi-Fi Protected Setup}
\acro{SMS}{Short message service}
\acro{REST}{Representational state transfer}
\acro{API}{Application Programming Interface}
\acro{TBS}{Transport block sizes}
\acro{VSBPP}{Variable Size Bin Packing Problem}
\acro{UART}{Universal Asynchronous Receiver/Transmitter}
\acro{SDN}{Software-defined networking}
\acro{CPS}{Cyber Physical System}
\acro{SFC}{Service Function Chaining}
\end{acronym}


==> Sections/approach_usecase.tex <==
%\subsection{Systematic Analysis}
%\noindent
For providing network resiliency in the Edge IoT network, we investigate the communication/connectivity  resiliency  of the end devices using  multi-mode communication.  


%There are three approaches here: top-down, bottom-up and a formal approach. In the top-down approach, data owners and associated parties provide their input on their perception of the multi-modal network resulting in the suitable use-cases. In the bottom-up approach, we focus on multi-modal communication first and understand the challenges (such as network and device limitations), resolve them to provide solutions to support the use cases. In the formal approach, the attributes of an application data flow, network are formally defined and based on the application and network availability, application data routes thru a particular network medium.
%The main aim of the project is to build data legibility and negotiability framework in multi-mode communication.  \py{Did we discuss data negotiability in abstract or conclusion? - this section needs rewriting please}
%There are three approaches here: top-down, bottom-up and a formal approach. In top-down, data owners and associated parties are taken into consideration and how they perceive/exercise control about the multi-modal network is taken into account. In the bottom-up approach, we focus on multi-modal communication first and understand the challenges, how to overcome these challenges to provide solutions which can be used to demonstrate the supporting use cases. In the formal approach, we describe the attributes of an application data flow which is further explained in \autoref{sec:system-model}. 

%In the bottom-up approach, At first, we understand the latency, data rates, number of messages limit per day available for each network medium. Based on that, we defined an application \appX which can utilise all network mediums. We aim to consider metrics such as latency, data rates of data transfer, throughput, payload size, security.%range (Distance), power, error-rates/inference effects, adaptiveness.
%  Furthermore, \lora, \nbiot, \sigfox have limits and latency, and our \appX application generates packets faster than \lora limits, we will explore and implement a queuing mechanism that introduces delay.

%The use case mentioned in \autoref{subsec:usecase} creates an interesting scenario where the end-user device (Pycom FiPy in our case) provides different network interfaces with a network specification such as bandwidth, latency, payload size, number of messages. Based on network characteristics, the different communication flows (via \lora/\sigfox/\nbiot/\wifi) are defined. On the other hand, data is categorised in terms of criticality (such as high/low priority), privacy settings, data length. Different profiles are implemented based on the data requirement, network suitability, and application scenario and the network traffic passes thru a particular communication flow. 

%The middleware can create a different type of profiles based on network availability and chooses the best one available at a given time based on the network conditions (bandwidth and latency of different networks and their availability (signal strength and coverage). The middleware shares information about the network status with the application. Based on the criticality of the message, the application decides the channel which would be utilised to send the data. As the network conditions changes, the application and the remote cloud is notified about the data source medium. We further explore from the perspective of data negotiability framework where multiple applications are running on the device, and the application decides not only from the technical network perspective but also from the privacy perspective. The privacy perspective can be that the user might not want to send data via \lora or \sigfox or public \wifi because of trust issues.  Networks can be defined as high risk or a low-risk network allowing users to define the security of the data and where it can be sent. In the scenario where the user does not define the privacy settings, they can be predefined based on understanding about application and data sensitivity.

%However, at the time of an emergency (for instance citizen having a heart attack), irrespective of the data security settings, based on the criticality of the data and urgency,  the middleware should override the security and privacy preferences and send the information with the best possible network. For example, connect to public \wifi or available network to ensure the information is sent to the hospital, emergency services as soon as possible. In a highly critical situation, the device may choose to break the fair usage policy of \lora, other networks and send the message.


%How is the local edge node smart enough to decide how to transfer packets? For example, currently, the node is not sending on \lora but able to connect \sigfox; so how quickly it adjusts its rate to choose \sigfox over \lora. How do we automate the process?

\subsection{Use-cases}
\label{subsec:usecase}
\noindent
LPWAN networks provide a fair use case for IoT applications having minimal computation and essential server communication. We explore a suitable use-case in the field of health analytics. Nowadays, there is an increased focus on continuous health monitoring, where a citizen has an IoT wearable device \appX monitoring heart rate, blood pressure at regular intervals. Further, the \appX provides a privacy-preserving setting configurable via GUI/mobile app in terms of data that can be shared and the frequency of uploads (per day/week/month) to the cloud server or hospital monitoring team. To provide an example, consider a citizen develops a health condition and needs medical attention and request a doctor appointment, the doctor requests for their past health condition recorded by the wearable device. The citizen can share the data with the hospital (for understanding past condition) via home \wifi remotely and avoid a visit to the hospital. The remote appointment saves money and time for the citizen as well as for the hospital. In the case of event-driven application, the \appX monitors the blood pressure, analyse, detect and report emergencies such as high blood pressure, irregular heartbeats. Such event-driven events would be one-time messages with the short payload.

Further, the above \appX can have a mobility feature where it can be indoor or outdoor.  In the scenario where the device running \appX is indoors, it could have functional connectivity over \wifi; however, signal strength for \lora, \sigfox, \nbiot could be inadequate, resulting in either limited or no connectivity for LPWAN networks.  As the connectivity indoors is with \wifi, the application can send the compressed data (in case of health, sending past one-month data at once) to the respective authorities. However, in the case of outdoors, the device might not have \wifi connectivity but have \lora, \sigfox, \nbiot connectivity as the signal quality is good outdoor than indoors. The user may choose to send selective data via LPWAN networks while outdoors. From the privacy perspective, the user can trust their home \wifi network rather than free \wifi available outdoors and can choose to define the type of data sent over a particular network interface. 

==> Sections/availablity.tex <==
\noindent
%We will make implementation code  open-source on github after paper acceptance. 
The implementation code is available online at \url{https://github.com/bitvijays/smartcity_multimode_networks} under  MIT license.

==> Sections/body.tex <==

Have sections and answer questions about 
\begin{itemize}
    \item Q1: Who supports the necessary public IoT infrastructure, and why? 
    \item Q2: Who will benefit from this infrastructure and what are the ethical, cultural, social, technical and economic barriers in achieving full benefit? 
    \item Q3: Who has access to the public space citizen data and how this data is going to be used? 
    \item Q4: What current mechanisms are used to take data usage consent from an end-user and how they are informed by other service users and providers that are involved in the whole ecosystem?
\end{itemize}
 
\subsection{Who supports the necessary public IoT infrastructure, and why?}

\notevk{Definition of Public IoT Infrastructure?}

These are mainly 

\begin{itemize}
    \item Government/ Regulation - Defra AURN?
    \item City-councils - Smart Barcelona
    \item Community Projects example - Smart Citizen Kit/ Luftdaten/ Organicity\footnote{\url{http://organicity.eu/}}
    \item Research-based Organisation/ Academia -- Examples Array of Things, Bristol is Open
\end{itemize}

\notevk{ Explain the above with examples}

\subsection{Who owns the infrastructure/ ecosystem?}

Sharing infrastructure or resources can result in multiple suppliers or service provider providing service to the customer as one entity. This service chain can further be breakdown to different vendors

\begin{itemize}
    \item Vendors who manage the applications and the hosting nodes at the edge/ cloud/ IoT platform.
    \item Vendors who own the sensors
    \item Vendors who manage those sensors
    \item Vendors who own the gateway, cloud
    \item Vendor offering connectivity between gateway and cloud (could be BT/ Vodafone).
\end{itemize}

It is a big ecosystem containing multiple vendors working together to deliver a service to the customer. 

\notevk{ Provide an example of the above scenario? If possible, real example.}

\subsection{Who will benefit from this infrastructure and what are the ethical, cultural, social, technical and economic barriers in achieving full benefit?}

\subsubsection{Who benefits from this infra}
\label{body:sss:benefit_infra}
\begin{itemize}
    \item Mainly government (releasing reports, meeting EU regulations directive ? Air Pollution standards, ensuring lockdown measures? COVID-19 etc.)
    \item Researchers? : Mention OneLab\footnote{\url{https://www.onelab.eu/}}? providing platform for researchers to deploy their custom applications? Developing models?
    \item Private Organisations: Organisation running transports ``First Bus''? or who want to know more about mobility of people.
    \item Citizens? Gathering open-source/ open-data? Awareness about their environment?
\end{itemize}

\subsubsection{what are the ethical, cultural, social, technical and economic barriers in achieving full benefit?}

\begin{itemize}
    \item Ethical: Mention details about London Face Recognition Pilot Study?
    \item Cultural: Find out If there's a cultural issue here? About gathering data? Citizens of China are used to a lot of data monitoring. However, UK people are quite against it? \notevk{Explore the area where citizen are happy to store/ transfer the data on BT network not on Huawei network}
    \item Social: Awareness maybe? For example: During HongKong protest, people attacked a few environment monitoring infra, thinking that the infra is doing Face recognition. Maybe a clear indication of running application on Infra would be better to avoid certain scenarios? (Transparency)?
    \item Technology? : Skilled resources? Technologies such as Kubernetes, Docker, LXC etc. are very fast-moving. With LF Edge Umbrella project, a lot of edge technologies moving very fast for a developer to keep up?
    \item Economic Barriers: City councils/ government stretched to be efficient? and cost-effective, doesn't have money until and unless benefits are very obvious?
\end{itemize}

\notevk{Expand the above with references}

\subsubsection{Who has access to the public space citizen data and how this data is going to be used?}

This might be repeated? Would be quite similar to subsubsection \ref{body:sss:benefit_infra}. Or we need to find more differences here.

\subsubsection{Q4: What current mechanisms are used to take data usage consent from an end-user and how they are informed by other service users and providers that are involved in the whole ecosystem?}

Probably, most of the public wouldn't be aware of the laws? For example: If people are putting a camera outside their house, what all stuff they can do? Or how long they are required/ can keep the feed? Can they do facial recognition on that feed? Or Count the number of pedestrians or not? 

\notevk{Maybe do a survey ? based on the number of questions on customer awareness on CCTV, InLinkUK or AoT and put up the results?}


==> Sections/planned_future_work.tex <==
# Short Paper Ideas and work

1. Fix UART issue of reading and writing messages too much by utilising Hardware Flow Control.
2. Include Payload message size, number of messages, security preferences into the CABFInv.
3. Include NBIoT integration + Pybytes + LtE-M
4. Explore event based programming in FiPy
5. Explore threads ? Why threads are not executing independently. 
6. Explore the introduction of Wi-Fi callback?
7. Explore how we can route LTE, WiFi altogether?
8. Why Sigfox, Lora not sending message altogether?
9. Instead of simulation of messages with random content, actually sending the sensor values? Check what different sensors can be attached to RPI? to simulate message flows?
10. Instead of accepting message just from UART, can we accept it from Wi-Fi too?

# Another extension
1. Add the Multi-resource management framework on the UAM architecture.




==> Tables/1_experiment_results.tex <==
\begin{table}[]
\makebox[0.48 \textwidth][c]{       %centering table
\resizebox{0.46 \textwidth}{!}{   %resize table

\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-12}
                                                                                               & \multicolumn{8}{c|}{\textbf{Message Flows}}                                                           & \multirow{\textbf{\begin{tabular}[c]{@{}c@{}}\% flows \\ served\end{tabular}}} & \multirow{\textbf{\begin{tabular}[c]{@{}c@{}}avg \\ crit\\ level\end{tabular}}} & \multirow{\textbf{objective}} \\ \cline{1-9}
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Allocation\\ algorithms\end{tabular}}} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} &                                                                                      &                                                                                              &                                                                \\ \hline
\multicolumn{1}{|l|}{L-FF}                                                                     & 1*         & 1*         & 1*         & 1*         & 1*         &            &            & 1*         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{L-FFD}                                                                    &            & 1\#       & 1\#        & 1*         & 1\#        & 1*         &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{H-FF}                                                                     & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{H-FFD}                                                                    & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{L-WF}                                                                     & 1*         & 1*         & 1*         & 1*         & 1*         &            &            & 1*         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{L-WFD}                                                                    &            & 1\#       & 1\#        & 1*         & 1\#        & 1*         &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{H-WF}                                                                     & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{H-WFD}                                                                    & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{L-BF}                                                                     & 1\#        & 1*         & 1+         & 1*         & 1\#        &            &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{L-BFD}                                                                    &            & 1\#       & 1+         & 1*         & 1\#        & 1*         &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{H-BF}                                                                     & 3+         & 3+         & 2+         & 2+         & 2+         & 2+         & 2+         & 1+         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{H-BFD}                                                                    & 3+         & 3+         & 2+         & 2+         & 2+         & 2+         & 2+         & 1+         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{CABF}                                                                     & 2+         & 1\#        & 1+         & 2+         & 1\#        & 1*         & 1*         & 1+         & 100                                                                                  & 1.25                                                                                         & 22                                  \\ \hline
\multicolumn{1}{|l|}{CABFinv}                                                                  & 1\#        & 2\#        & 1+         & 2+         & 1\#        & 1*         & 1*         & 1+         & 100                                                                                  & 1.25                                                                                         & 22                                  \\ \hline
\multicolumn{1}{|l|}{Optimal}                                                                  & 1*         & 1*         & 1*         & 1*         & 1*         & 2*         & 2*         & 1*         & 100                                                                                  & 1.25                                                                                         & 22                                  \\ \hline
\end{tabular}

} %close resize
} %close centering
\caption{Obtained criticality level (1 | 2 | 3) and network allocation (* Wi-Fi | \# Lora | + Sigfox) for motivating example.}
\label{tab:AssistedLivingExampleResults}
\end{table}

==> Tables/1_experiment_results2.tex <==
\begin{table}[]
\makebox[0.48 \textwidth][c]{       %centering table
\resizebox{0.47 \textwidth}{!}{   %resize table

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-12}
\textbf{} & \multicolumn{8}{c|}{\textbf{Message Flows}} & \multirow{\textbf{\begin{tabular}[c]{@{}c@{}}\% flows \\ served\end{tabular}}} & \multirow{\textbf{\begin{tabular}[c]{@{}c@{}}avg \\ crit\\ level\end{tabular}}} & \multirow{\textbf{objective}} \\ \cline{2-9}
    & 1 & 2 & 3 & 4 & 5    & 6    & 7    & 8    &   & &                                     \\ \cline{1-9}
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Requested \\ crit level\end{tabular}}} & 1,2,3  & 1,2,3  & 1,2  & 1,2  & 1,2  & 1,2  & 1,2  & 1    &                                          &                                                 &                                     \\ \cline{1-9}
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}l@{}}Allocation\\ algorithms\end{tabular}}}       & \multicolumn{8}{c|}{\textbf{Allocated Criticality Level}}                                     &                                          &                                                 &                                     \\ \hline
\multicolumn{1}{|l|}{L-FF}                                                                     & 1*         & 1*         & 1*         & 1*         & 1*         &            &            & 1*         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{L-FFD}                                                                    &            & 1\#       & 1\#        & 1*         & 1\#        & 1*         &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{H-FF}                                                                     & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{H-FFD}                                                                    & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{L-WF}                                                                     & 1*         & 1*         & 1*         & 1*         & 1*         &            &            & 1*         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{L-WFD}                                                                    &            & 1\#       & 1\#        & 1*         & 1\#        & 1*         &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{H-WF}                                                                     & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{H-WFD}                                                                    & 3*         & 3*         & 2*         & 2*         & 2*         & 2*         & 2*         & 1*         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{L-BF}                                                                     & 1\#        & 1*         & 1+         & 1*         & 1\#        &            &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{L-BFD}                                                                    &            & 1\#       & 1+         & 1*         & 1\#        & 1*         &            & 1+         & 75                                                                                   & 1                                                                                            & 18                                  \\ \hline
\multicolumn{1}{|l|}{H-BF}                                                                     & 3+         & 3+         & 2+         & 2+         & 2+         & 2+         & 2+         & 1+         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{H-BFD}                                                                    & 3+         & 3+         & 2+         & 2+         & 2+         & 2+         & 2+         & 1+         & 100                                                                                  & 2.12                                                                                         & 15                                  \\ \hline
\multicolumn{1}{|l|}{CABF}                                                                     & 2+         & 1\#        & 1+         & 2+         & 1\#        & 1*         & 1*         & 1+         & 100                                                                                  & 1.25                                                                                         & 22                                  \\ \hline
\multicolumn{1}{|l|}{CABFinv}                                                                  & 1\#        & 2\#        & 1+         & 2+         & 1\#        & 1*         & 1*         & 1+         & 100                                                                                  & 1.25                                                                                         & 22                                  \\ \hline
\multicolumn{1}{|l|}{Optimal}                                                                  & 1*         & 1*         & 1*         & 1*         & 1*         & 2*         & 2*         & 1*         & 100                                                                                  & 1.25                                                                                         & 22                                  \\ \hline
\end{tabular}

} %close resize
} %close centering
\caption{Obtained criticality level (1 | 2 | 3) and network allocation (* Wi-Fi | \# Lora | + Sigfox) for motivating example.}
\label{tab:AssistedLivingExampleResults}
\end{table}

==> Tables/baseline_summary.tex <==
\begin{table*}

\makebox[1 \textwidth][c]{     %centering table
\resizebox{1 \textwidth}{!}{   %resize table

\centering

\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Baseline}          & \textbf{LoRaWAN}                      & \textbf{SigFox}    & \textbf{NB-IoT}                                                               & \textbf{Wi-Fi}                                      \\ \hline
Max-Payload Length         & 1 - 222 bytes                         & 1-12 bytes         & UDP/TCP/IP                                                                    & UDP/TCP/IP                                          \\ \hline
Sending Continuous Data     & 0.165ms                               & 10.5 seconds       & Few ms                                                                        & Few ms                                              \\ \hline
Latency                    & 24-2800ms + few seconds               & 1 - 4.5 sec        & 500 ms (avg)                                                                  & 8 ms (avg)                                          \\ \hline
Throughput                 & 250 - 11000 bps                       & 100 UL/ 600 DL bps & NB-IoT: 26 kbps DL/ 66Kbps UL; LTE-M: 300kbps DL/ 380 kbps; Avg: 100-150 kbps & 3550 kbps (local machine) 770 kbps (remote machine) \\ \hline
Time to connect to network & OTAA:5.6 sec/ ABP (join not required) & few ms             & With LTE Reset: 20 sec | Without LTE Reset: 15.5 sec                          & 7.7 sec                                             \\ \hline
\end{tabular}
} %close resize
} %close centering
\caption{Baseline metrics Summary.}
\label{tab:baseline_summary}
\end{table*}

==> Tables/sigfox_real.tex <==
\begin{table}[]
\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Payload Length} & \textbf{Average (sec)} & \textbf{Good/Excellent (sec)}\\ \hline
%\textless{}1 bit        & 1.1\\ \hline
2 bit - 1 byte          & 1.6 & 2\\ \hline
2-4 byte                & 2.3 & 2.1\\ \hline
5-8 byte                & 4.5 & 2.5\\ \hline
9-12 byte               & 4.5 & 3\\ \hline
\end{tabular}
\end{adjustbox}
\caption{Real \sigfox Payload time for Average, Good/Excellent Quality for RC1.}
\label{tab:sigfox-payloadtime-real}
\end{table}

==> Tables/sigfox_tech.tex <==
\begin{table}[]
\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Payload Length} & \textbf{Theoretical} & \textbf{Average} & \textbf{Good/Excellent}\\ \hline
\textless{}1 bit        & 1.1                        & 190           \\ \hline
2 bit - 1 byte          & 1.2                        & 1.6 & 2.0        \\ \hline
2-4 byte                & 1.45                       & 2.3 & 2.1        \\ \hline
5-8 byte                & 1.75                       & 4.5 & 2.5          \\ \hline
9-12 byte               & 2                          & 4.5 & 3            \\ \hline
\end{tabular}
\end{adjustbox}
\caption{\sigfox Payload time Theoretical vs Measured for Average, Good/Excellent Quality at RC1 Region.}
\label{tab:sigfox-payloadtime-tech}
\end{table}

==> plot/Raw_Data/lora_connect.tex <==
2020-08-17 02:47:07InitTime:0,JoinTime7,sock_time4,send_Time0
2020-08-17 02:48:14InitTime:0,JoinTime7,sock_time4,send_Time0
2020-08-17 02:52:31InitTime:0,JoinTime7,sock_time0,send_Time0
2020-08-17 02:55:37InitTime:0,JoinTime8,sock_time0,send_Time0
2020-08-17 02:55:52InitTime:0,JoinTime8,sock_time0,send_Time0
2020-08-17 02:56:07InitTime:0,JoinTime8,sock_time0,send_Time0
2020-08-17 02:56:12InitTime:0,JoinTime2,sock_time0,send_Time0
2020-08-17 02:56:39InitTime:0,JoinTime8,sock_time0,send_Time0
2020-08-17 02:56:44InitTime:0,JoinTime2,sock_time0,send_Time0
2020-08-17 02:56:54InitTime:0,JoinTime3,sock_time0,send_Time0
2020-08-17 02:57:50InitTime:0,JoinTime7,sock_time0,send_Time0
2020-08-17 03:02:40InitTime:0,JoinTime7,sock_time0,send_Time0
2020-08-17 03:03:51InitTime:0,JoinTime8,sock_time0,send_Time0
1970-01-01 01:00:21InitTime:0,JoinTime7,sock_time0,send_Time0
1970-01-01 01:04:46InitTime:0,JoinTime8,sock_time0,send_Time0
2020-08-17 03:18:31InitTime:0,JoinTime8,sock_time0,send_Time0
2020-08-17 03:18:12InitTime:0,JoinTime7,sock_time0,send_Time0
2020-08-17 03:27:08,InitTime:0,JoinTime:7,sock_time:0,send_Time:0
2020-08-17 03:27:13,InitTime:0,JoinTime:5,sock_time:0,send_Time:0
2020-08-17 03:27:19,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:27:23,InitTime:0,JoinTime:4,sock_time:0,send_Time:0
2020-08-17 03:27:29,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:27:33,InitTime:0,JoinTime:4,sock_time:0,send_Time:0
2020-08-17 03:27:39,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:33:45,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:33:50,InitTime:0,JoinTime:5,sock_time:0,send_Time:0
2020-08-17 03:33:56,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:34:00,InitTime:0,JoinTime:4,sock_time:0,send_Time:0
2020-08-17 03:34:06,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:34:10,InitTime:0,JoinTime:4,sock_time:0,send_Time:0
2020-08-17 03:34:16,InitTime:0,JoinTime:6,sock_time:0,send_Time:0
2020-08-17 03:37:43,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:40:13,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:40:41,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:41:19,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:41:48,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:42:23,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:43:48,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:44:19,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:45:10,InitTime:0,JoinTime:6,sock_time:0,send_Time:5
2020-08-17 03:47:09,InitTime:0,JoinTime:6,sock_time:0,send_Time:5



SF12

2020-08-17 21:45:29,InitTime:0,JoinTime:10,sock_time:0,send_Time:0
2020-08-17 21:45:34,InitTime:0,JoinTime:5,sock_time:0,send_Time:0
2020-08-17 21:45:49,InitTime:0,JoinTime:10,sock_time:0,send_Time:0
2020-08-17 21:46:03,InitTime:0,JoinTime:9,sock_time:0,send_Time:0
2020-08-17 21:40:00,InitTime:0,JoinTime:10,sock_time:0,send_Time:0
2020-08-17 21:40:05,InitTime:0,JoinTime:5,sock_time:0,send_Time:0
2020-08-17 21:40:15,InitTime:0,JoinTime:10,sock_time:0,send_Time:0
2020-08-17 21:40:20,InitTime:0,JoinTime:5,sock_time:0,send_Time:0
2020-08-17 21:40:30,InitTime:0,JoinTime:10,sock_time:0,send_Time:0
2020-08-17 21:40:34,InitTime:0,JoinTime:4,sock_time:0,send_Time:0
2020-08-17 21:40:44,InitTime:0,JoinTime:10,sock_time:0,send_Time:0

==> plot/Raw_Data/lte_latency.tex <==
>>> import uping
>>> uping.ping('10.200.0.1')
PING 10.200.0.1 (10.200.0.1): 64 data bytes
84 bytes from 10.200.0.1: icmp_seq=9, ttl=252, time=14926.564693 ms
84 bytes from 10.200.0.1: icmp_seq=10, ttl=252, time=14146.156311 ms
84 bytes from 10.200.0.1: icmp_seq=12, ttl=252, time=12174.040079 ms
84 bytes from 10.200.0.1: icmp_seq=14, ttl=252, time=10330.163240 ms
84 bytes from 10.200.0.1: icmp_seq=16, ttl=252, time=8359.141350 ms
84 bytes from 10.200.0.1: icmp_seq=17, ttl=252, time=7579.204082 ms
84 bytes from 10.200.0.1: icmp_seq=18, ttl=252, time=6610.110760 ms
84 bytes from 10.200.0.1: icmp_seq=19, ttl=252, time=5765.246868 ms
84 bytes from 10.200.0.1: icmp_seq=20, ttl=252, time=4826.081276 ms
84 bytes from 10.200.0.1: icmp_seq=21, ttl=252, time=4050.395966 ms
84 bytes from 10.200.0.1: icmp_seq=22, ttl=252, time=3011.847019 ms
84 bytes from 10.200.0.1: icmp_seq=23, ttl=252, time=2168.246984 ms
84 bytes from 10.200.0.1: icmp_seq=24, ttl=252, time=1191.215878 ms
84 bytes from 10.200.0.1: icmp_seq=25, ttl=252, time=333.302999 ms
84 bytes from 10.200.0.1: icmp_seq=26, ttl=252, time=467.388010 ms
84 bytes from 10.200.0.1: icmp_seq=27, ttl=252, time=740.031958 ms
84 bytes from 10.200.0.1: icmp_seq=28, ttl=252, time=370.785999 ms
84 bytes from 10.200.0.1: icmp_seq=29, ttl=252, time=639.816999 ms
84 bytes from 10.200.0.1: icmp_seq=30, ttl=252, time=271.818995 ms
84 bytes from 10.200.0.1: icmp_seq=31, ttl=252, time=532.841015 ms
84 bytes from 10.200.0.1: icmp_seq=32, ttl=252, time=801.729965 ms
84 bytes from 10.200.0.1: icmp_seq=33, ttl=252, time=427.833986 ms
84 bytes from 10.200.0.1: icmp_seq=34, ttl=252, time=697.737980 ms
84 bytes from 10.200.0.1: icmp_seq=35, ttl=252, time=329.821014 ms
84 bytes from 10.200.0.1: icmp_seq=36, ttl=252, time=599.773979 ms
84 bytes from 10.200.0.1: icmp_seq=37, ttl=252, time=869.837952 ms
84 bytes from 10.200.0.1: icmp_seq=38, ttl=252, time=501.829004 ms
84 bytes from 10.200.0.1: icmp_seq=39, ttl=252, time=771.807003 ms
84 bytes from 10.200.0.1: icmp_seq=40, ttl=252, time=403.706980 ms
84 bytes from 10.200.0.1: icmp_seq=41, ttl=252, time=670.773983 ms
84 bytes from 10.200.0.1: icmp_seq=42, ttl=252, time=347.770977 ms
84 bytes from 10.200.0.1: icmp_seq=43, ttl=252, time=502.228975 ms
84 bytes from 10.200.0.1: icmp_seq=44, ttl=252, time=774.583960 ms
84 bytes from 10.200.0.1: icmp_seq=45, ttl=252, time=406.190014 ms
84 bytes from 10.200.0.1: icmp_seq=46, ttl=252, time=676.496983 ms
84 bytes from 10.200.0.1: icmp_seq=47, ttl=252, time=304.582000 ms
84 bytes from 10.200.0.1: icmp_seq=48, ttl=252, time=574.891996 ms
84 bytes from 10.200.0.1: icmp_seq=49, ttl=252, time=843.782997 ms
84 bytes from 10.200.0.1: icmp_seq=50, ttl=252, time=475.775003 ms
50 packets transmitted, 39 packets received

>>> uping.ping('10.200.0.1')
PING 10.200.0.1 (10.200.0.1): 64 data bytes
84 bytes from 10.200.0.1: icmp_seq=1, ttl=252, time=8326.947212 ms
84 bytes from 10.200.0.1: icmp_seq=2, ttl=252, time=9032.845497 ms
84 bytes from 10.200.0.1: icmp_seq=4, ttl=252, time=7522.737980 ms
84 bytes from 10.200.0.1: icmp_seq=6, ttl=252, time=6235.660076 ms
84 bytes from 10.200.0.1: icmp_seq=8, ttl=252, time=5433.793068 ms
84 bytes from 10.200.0.1: icmp_seq=9, ttl=252, time=4748.702049 ms
84 bytes from 10.200.0.1: icmp_seq=10, ttl=252, time=4015.659809 ms
84 bytes from 10.200.0.1: icmp_seq=11, ttl=252, time=4122.591972 ms
84 bytes from 10.200.0.1: icmp_seq=12, ttl=252, time=3454.579115 ms
84 bytes from 10.200.0.1: icmp_seq=13, ttl=252, time=2604.408026 ms
84 bytes from 10.200.0.1: icmp_seq=14, ttl=252, time=1842.620850 ms
84 bytes from 10.200.0.1: icmp_seq=15, ttl=252, time=1331.760049 ms
84 bytes from 10.200.0.1: icmp_seq=16, ttl=252, time=759.814024 ms
84 bytes from 10.200.0.1: icmp_seq=17, ttl=252, time=568.431997 ms
84 bytes from 10.200.0.1: icmp_seq=18, ttl=252, time=831.748962 ms
84 bytes from 10.200.0.1: icmp_seq=19, ttl=252, time=1156.663895 ms
84 bytes from 10.200.0.1: icmp_seq=20, ttl=252, time=533.797979 ms
84 bytes from 10.200.0.1: icmp_seq=21, ttl=252, time=1937.176895 ms
84 bytes from 10.200.0.1: icmp_seq=22, ttl=252, time=1265.262961 ms
84 bytes from 10.200.0.1: icmp_seq=23, ttl=252, time=796.449995 ms
84 bytes from 10.200.0.1: icmp_seq=24, ttl=252, time=850.687981 ms
84 bytes from 10.200.0.1: icmp_seq=25, ttl=252, time=886.312962 ms
84 bytes from 10.200.0.1: icmp_seq=26, ttl=252, time=1054.369926 ms
84 bytes from 10.200.0.1: icmp_seq=27, ttl=252, time=500.771999 ms
84 bytes from 10.200.0.1: icmp_seq=28, ttl=252, time=955.807972 ms
84 bytes from 10.200.0.1: icmp_seq=29, ttl=252, time=655.885983 ms
84 bytes from 10.200.0.1: icmp_seq=30, ttl=252, time=811.846924 ms
84 bytes from 10.200.0.1: icmp_seq=31, ttl=252, time=1081.745987 ms
84 bytes from 10.200.0.1: icmp_seq=32, ttl=252, time=486.770964 ms
84 bytes from 10.200.0.1: icmp_seq=33, ttl=252, time=939.828014 ms
84 bytes from 10.200.0.1: icmp_seq=34, ttl=252, time=678.809977 ms
84 bytes from 10.200.0.1: icmp_seq=35, ttl=252, time=841.849995 ms
84 bytes from 10.200.0.1: icmp_seq=36, ttl=252, time=485.785007 ms
84 bytes from 10.200.0.1: icmp_seq=37, ttl=252, time=757.894993 ms
84 bytes from 10.200.0.1: icmp_seq=38, ttl=252, time=1027.587056 ms
84 bytes from 10.200.0.1: icmp_seq=39, ttl=252, time=387.821007 ms
84 bytes from 10.200.0.1: icmp_seq=40, ttl=252, time=895.798969 ms
84 bytes from 10.200.0.1: icmp_seq=41, ttl=252, time=527.752018 ms
84 bytes from 10.200.0.1: icmp_seq=42, ttl=252, time=798.687983 ms
84 bytes from 10.200.0.1: icmp_seq=43, ttl=252, time=970.273018 ms
84 bytes from 10.200.0.1: icmp_seq=44, ttl=252, time=741.364956 ms
84 bytes from 10.200.0.1: icmp_seq=45, ttl=252, time=871.749020 ms
84 bytes from 10.200.0.1: icmp_seq=46, ttl=252, time=504.266977 ms
84 bytes from 10.200.0.1: icmp_seq=47, ttl=252, time=772.343969 ms
84 bytes from 10.200.0.1: icmp_seq=48, ttl=252, time=404.660988 ms
84 bytes from 10.200.0.1: icmp_seq=49, ttl=252, time=813.797951 ms
84 bytes from 10.200.0.1: icmp_seq=50, ttl=252, time=785.718966 ms
50 packets transmitted, 47 packets received

PING 10.200.0.1 (10.200.0.1): 64 data bytes
84 bytes from 10.200.0.1: icmp_seq=1, ttl=252, time=1339.954019 ms
84 bytes from 10.200.0.1: icmp_seq=2, ttl=252, time=529.456949 ms
84 bytes from 10.200.0.1: icmp_seq=3, ttl=252, time=539.911985 ms
84 bytes from 10.200.0.1: icmp_seq=4, ttl=252, time=809.838963 ms
84 bytes from 10.200.0.1: icmp_seq=5, ttl=252, time=442.022991 ms
84 bytes from 10.200.0.1: icmp_seq=6, ttl=252, time=640.405989 ms
84 bytes from 10.200.0.1: icmp_seq=7, ttl=252, time=269.503999 ms
84 bytes from 10.200.0.1: icmp_seq=8, ttl=252, time=541.939974 ms
84 bytes from 10.200.0.1: icmp_seq=9, ttl=252, time=813.206959 ms
84 bytes from 10.200.0.1: icmp_seq=10, ttl=252, time=444.359970 ms
84 bytes from 10.200.0.1: icmp_seq=11, ttl=252, time=713.879013 ms
84 bytes from 10.200.0.1: icmp_seq=12, ttl=252, time=345.770979 ms
84 bytes from 10.200.0.1: icmp_seq=13, ttl=252, time=615.791988 ms
84 bytes from 10.200.0.1: icmp_seq=14, ttl=252, time=245.738006 ms










>> uping.ping('10.200.0.1')
PING 10.200.0.1 (10.200.0.1): 64 data bytes
84 bytes from 10.200.0.1: icmp_seq=1, ttl=252, time=9854.789734 ms
84 bytes from 10.200.0.1: icmp_seq=2, ttl=252, time=9075.848579 ms
84 bytes from 10.200.0.1: icmp_seq=4, ttl=252, time=7101.016521 ms
84 bytes from 10.200.0.1: icmp_seq=6, ttl=252, time=5254.251003 ms
84 bytes from 10.200.0.1: icmp_seq=8, ttl=252, time=3281.869888 ms
84 bytes from 10.200.0.1: icmp_seq=10, ttl=252, time=1483.660126 ms
84 bytes from 10.200.0.1: icmp_seq=11, ttl=252, time=520.260000 ms
84 bytes from 10.200.0.1: icmp_seq=12, ttl=252, time=711.752987 ms
84 bytes from 10.200.0.1: icmp_seq=13, ttl=252, time=343.863010 ms
84 bytes from 10.200.0.1: icmp_seq=14, ttl=252, time=612.851000 ms
84 bytes from 10.200.0.1: icmp_seq=15, ttl=252, time=881.671047 ms
84 bytes from 10.200.0.1: icmp_seq=16, ttl=252, time=510.834980 ms
84 bytes from 10.200.0.1: icmp_seq=17, ttl=252, time=782.223988 ms
84 bytes from 10.200.0.1: icmp_seq=18, ttl=252, time=411.788988 ms
84 bytes from 10.200.0.1: icmp_seq=19, ttl=252, time=682.741022 ms
84 bytes from 10.200.0.1: icmp_seq=20, ttl=252, time=313.765979 ms
84 bytes from 10.200.0.1: icmp_seq=21, ttl=252, time=584.161997 ms
84 bytes from 10.200.0.1: icmp_seq=22, ttl=252, time=788.245964 ms
84 bytes from 10.200.0.1: icmp_seq=23, ttl=252, time=418.389988 ms
84 bytes from 10.200.0.1: icmp_seq=24, ttl=252, time=689.369011 ms
84 bytes from 10.200.0.1: icmp_seq=25, ttl=252, time=318.303013 ms
84 bytes from 10.200.0.1: icmp_seq=26, ttl=252, time=587.391996 ms
84 bytes from 10.200.0.1: icmp_seq=27, ttl=252, time=860.791016 ms
84 bytes from 10.200.0.1: icmp_seq=28, ttl=252, time=489.969969 ms
84 bytes from 10.200.0.1: icmp_seq=29, ttl=252, time=759.806967 ms
84 bytes from 10.200.0.1: icmp_seq=30, ttl=252, time=392.372017 ms
84 bytes from 10.200.0.1: icmp_seq=31, ttl=252, time=661.870956 ms
84 bytes from 10.200.0.1: icmp_seq=32, ttl=252, time=293.780994 ms
84 bytes from 10.200.0.1: icmp_seq=33, ttl=252, time=561.749029 ms
84 bytes from 10.200.0.1: icmp_seq=34, ttl=252, time=832.824993 ms
84 bytes from 10.200.0.1: icmp_seq=35, ttl=252, time=461.988020 ms
84 bytes from 10.200.0.1: icmp_seq=36, ttl=252, time=733.815002 ms
84 bytes from 10.200.0.1: icmp_seq=37, ttl=252, time=363.759995 ms
84 bytes from 10.200.0.1: icmp_seq=38, ttl=252, time=633.745956 ms
84 bytes from 10.200.0.1: icmp_seq=39, ttl=252, time=265.821981 ms
84 bytes from 10.200.0.1: icmp_seq=40, ttl=252, time=536.770964 ms
84 bytes from 10.200.0.1: icmp_seq=41, ttl=252, time=806.825924 ms
84 bytes from 10.200.0.1: icmp_seq=42, ttl=252, time=437.641001 ms
84 bytes from 10.200.0.1: icmp_seq=43, ttl=252, time=638.346004 ms
84 bytes from 10.200.0.1: icmp_seq=44, ttl=252, time=271.934986 ms
84 bytes from 10.200.0.1: icmp_seq=45, ttl=252, time=544.315958 ms
84 bytes from 10.200.0.1: icmp_seq=46, ttl=252, time=2781.782866 ms
84 bytes from 10.200.0.1: icmp_seq=47, ttl=252, time=1810.930157 ms
84 bytes from 10.200.0.1: icmp_seq=48, ttl=252, time=942.202950 ms
84 bytes from 10.200.0.1: icmp_seq=49, ttl=252, time=337.785006 ms
84 bytes from 10.200.0.1: icmp_seq=50, ttl=252, time=608.027983 ms
84 bytes from 10.200.0.1: icmp_seq=51, ttl=252, time=879.814053 ms
84 bytes from 10.200.0.1: icmp_seq=52, ttl=252, time=509.894991 ms
84 bytes from 10.200.0.1: icmp_seq=53, ttl=252, time=780.814981 ms
84 bytes from 10.200.0.1: icmp_seq=54, ttl=252, time=411.198997 ms
84 bytes from 10.200.0.1: icmp_seq=55, ttl=252, time=680.806017 ms
84 bytes from 10.200.0.1: icmp_seq=56, ttl=252, time=311.838984 ms
84 bytes from 10.200.0.1: icmp_seq=57, ttl=252, time=581.898975 ms
84 bytes from 10.200.0.1: icmp_seq=58, ttl=252, time=852.744961 ms
84 bytes from 10.200.0.1: icmp_seq=59, ttl=252, time=481.797981 ms
84 bytes from 10.200.0.1: icmp_seq=60, ttl=252, time=754.138947 ms
84 bytes from 10.200.0.1: icmp_seq=61, ttl=252, time=383.782978 ms
84 bytes from 10.200.0.1: icmp_seq=62, ttl=252, time=653.762007 ms
84 bytes from 10.200.0.1: icmp_seq=63, ttl=252, time=283.799000 ms
84 bytes from 10.200.0.1: icmp_seq=64, ttl=252, time=487.276983 ms
84 bytes from 10.200.0.1: icmp_seq=65, ttl=252, time=755.393982 ms
84 bytes from 10.200.0.1: icmp_seq=66, ttl=252, time=387.334013 ms
84 bytes from 10.200.0.1: icmp_seq=67, ttl=252, time=658.306026 ms
84 bytes from 10.200.0.1: icmp_seq=68, ttl=252, time=290.279980 ms
84 bytes from 10.200.0.1: icmp_seq=69, ttl=252, time=560.900974 ms
84 bytes from 10.200.0.1: icmp_seq=70, ttl=252, time=831.697941 ms
84 bytes from 10.200.0.1: icmp_seq=71, ttl=252, time=459.931993 ms
84 bytes from 10.200.0.1: icmp_seq=72, ttl=252, time=731.745958 ms
84 bytes from 10.200.0.1: icmp_seq=73, ttl=252, time=361.803007 ms
84 bytes from 10.200.0.1: icmp_seq=74, ttl=252, time=631.903982 ms
84 bytes from 10.200.0.1: icmp_seq=75, ttl=252, time=263.795996 ms
84 bytes from 10.200.0.1: icmp_seq=76, ttl=252, time=533.801985 ms
84 bytes from 10.200.0.1: icmp_seq=77, ttl=252, time=850.767994 ms
84 bytes from 10.200.0.1: icmp_seq=78, ttl=252, time=427.801991 ms
84 bytes from 10.200.0.1: icmp_seq=79, ttl=252, time=699.754000 ms
84 bytes from 10.200.0.1: icmp_seq=80, ttl=252, time=330.267000 ms
84 bytes from 10.200.0.1: icmp_seq=81, ttl=252, time=599.755001 ms
84 bytes from 10.200.0.1: icmp_seq=82, ttl=252, time=869.775963 ms
84 bytes from 10.200.0.1: icmp_seq=83, ttl=252, time=501.823997 ms
84 bytes from 10.200.0.1: icmp_seq=84, ttl=252, time=772.620964 ms
84 bytes from 10.200.0.1: icmp_seq=85, ttl=252, time=335.993004 ms
84 bytes from 10.200.0.1: icmp_seq=86, ttl=252, time=605.366993 ms
84 bytes from 10.200.0.1: icmp_seq=87, ttl=252, time=878.308010 ms
84 bytes from 10.200.0.1: icmp_seq=88, ttl=252, time=508.368015 ms
84 bytes from 10.200.0.1: icmp_seq=89, ttl=252, time=779.601955 ms
84 bytes from 10.200.0.1: icmp_seq=90, ttl=252, time=410.243988 ms
84 bytes from 10.200.0.1: icmp_seq=91, ttl=252, time=680.171013 ms
84 bytes from 10.200.0.1: icmp_seq=92, ttl=252, time=311.774993 ms
84 bytes from 10.200.0.1: icmp_seq=93, ttl=252, time=583.723021 ms
84 bytes from 10.200.0.1: icmp_seq=94, ttl=252, time=853.754044 ms
84 bytes from 10.200.0.1: icmp_seq=95, ttl=252, time=482.881975 ms
84 bytes from 10.200.0.1: icmp_seq=96, ttl=252, time=753.741980 ms
84 bytes from 10.200.0.1: icmp_seq=97, ttl=252, time=383.724995 ms
84 bytes from 10.200.0.1: icmp_seq=98, ttl=252, time=656.754971 ms
84 bytes from 10.200.0.1: icmp_seq=99, ttl=252, time=285.834980 ms
84 bytes from 10.200.0.1: icmp_seq=100, ttl=252, time=555.760956 ms
84 bytes from 10.200.0.1: icmp_seq=101, ttl=252, time=827.952957 ms
84 bytes from 10.200.0.1: icmp_seq=102, ttl=252, time=459.286976 ms
84 bytes from 10.200.0.1: icmp_seq=103, ttl=252, time=727.696991 ms
84 bytes from 10.200.0.1: icmp_seq=104, ttl=252, time=357.747006 ms
84 bytes from 10.200.0.1: icmp_seq=105, ttl=252, time=728.242970 ms
84 bytes from 10.200.0.1: icmp_seq=106, ttl=252, time=829.146957 ms
84 bytes from 10.200.0.1: icmp_seq=107, ttl=252, time=457.253981 ms
84 bytes from 10.200.0.1: icmp_seq=108, ttl=252, time=728.357935 ms
84 bytes from 10.200.0.1: icmp_seq=109, ttl=252, time=361.342978 ms
84 bytes from 10.200.0.1: icmp_seq=110, ttl=252, time=631.383944 ms
84 bytes from 10.200.0.1: icmp_seq=111, ttl=252, time=264.175987 ms
84 bytes from 10.200.0.1: icmp_seq=112, ttl=252, time=538.643980 ms
84 bytes from 10.200.0.1: icmp_seq=113, ttl=252, time=805.751991 ms
84 bytes from 10.200.0.1: icmp_seq=114, ttl=252, time=437.828016 ms
84 bytes from 10.200.0.1: icmp_seq=115, ttl=252, time=708.263969 ms
84 bytes from 10.200.0.1: icmp_seq=116, ttl=252, time=339.911985 ms
84 bytes from 10.200.0.1: icmp_seq=117, ttl=252, time=609.770966 ms
84 bytes from 10.200.0.1: icmp_seq=118, ttl=252, time=881.742954 ms
84 bytes from 10.200.0.1: icmp_seq=119, ttl=252, time=509.733009 ms
84 bytes from 10.200.0.1: icmp_seq=120, ttl=252, time=780.841970 ms
84 bytes from 10.200.0.1: icmp_seq=121, ttl=252, time=411.768007 ms
84 bytes from 10.200.0.1: icmp_seq=122, ttl=252, time=681.814003 ms
84 bytes from 10.200.0.1: icmp_seq=123, ttl=252, time=359.810996 ms
84 bytes from 10.200.0.1: icmp_seq=124, ttl=252, time=583.786964 ms
84 bytes from 10.200.0.1: icmp_seq=125, ttl=252, time=853.783035 ms
84 bytes from 10.200.0.1: icmp_seq=126, ttl=252, time=485.967016 ms
84 bytes from 10.200.0.1: icmp_seq=127, ttl=252, time=688.469934 ms
84 bytes from 10.200.0.1: icmp_seq=128, ttl=252, time=317.364979 ms
84 bytes from 10.200.0.1: icmp_seq=129, ttl=252, time=588.225985 ms
84 bytes from 10.200.0.1: icmp_seq=130, ttl=252, time=859.372997 ms
84 bytes from 10.200.0.1: icmp_seq=131, ttl=252, time=490.344000 ms
84 bytes from 10.200.0.1: icmp_seq=132, ttl=252, time=761.319971 ms
84 bytes from 10.200.0.1: icmp_seq=133, ttl=252, time=392.765980 ms
84 bytes from 10.200.0.1: icmp_seq=134, ttl=252, time=661.776972 ms
84 bytes from 10.200.0.1: icmp_seq=135, ttl=252, time=291.800995 ms
84 bytes from 10.200.0.1: icmp_seq=136, ttl=252, time=563.757992 ms
84 bytes from 10.200.0.1: icmp_seq=137, ttl=252, time=833.745956 ms
84 bytes from 10.200.0.1: icmp_seq=138, ttl=252, time=465.786982 ms
84 bytes from 10.200.0.1: icmp_seq=139, ttl=252, time=736.801004 ms
84 bytes from 10.200.0.1: icmp_seq=140, ttl=252, time=365.836000 ms
84 bytes from 10.200.0.1: icmp_seq=141, ttl=252, time=637.840033 ms
84 bytes from 10.200.0.1: icmp_seq=142, ttl=252, time=291.735983 ms
84 bytes from 10.200.0.1: icmp_seq=143, ttl=252, time=530.882025 ms
84 bytes from 10.200.0.1: icmp_seq=144, ttl=252, time=801.780987 ms
84 bytes from 10.200.0.1: icmp_seq=145, ttl=252, time=431.764984 ms
84 bytes from 10.200.0.1: icmp_seq=146, ttl=252, time=703.856993 ms
84 bytes from 10.200.0.1: icmp_seq=147, ttl=252, time=333.744979 ms
84 bytes from 10.200.0.1: icmp_seq=148, ttl=252, time=539.460993 ms
84 bytes from 10.200.0.1: icmp_seq=149, ttl=252, time=808.286953 ms
84 bytes from 10.200.0.1: icmp_seq=150, ttl=252, time=438.590002 ms
84 bytes from 10.200.0.1: icmp_seq=151, ttl=252, time=707.718992 ms
84 bytes from 10.200.0.1: icmp_seq=152, ttl=252, time=338.502002 ms
84 bytes from 10.200.0.1: icmp_seq=153, ttl=252, time=607.333994 ms
84 bytes from 10.200.0.1: icmp_seq=154, ttl=252, time=878.754997 ms
84 bytes from 10.200.0.1: icmp_seq=155, ttl=252, time=507.701969 ms
84 bytes from 10.200.0.1: icmp_seq=156, ttl=252, time=779.762983 ms
84 bytes from 10.200.0.1: icmp_seq=157, ttl=252, time=409.863997 ms
84 bytes from 10.200.0.1: icmp_seq=158, ttl=252, time=681.767988 ms
84 bytes from 10.200.0.1: icmp_seq=159, ttl=252, time=311.778975 ms
84 bytes from 10.200.0.1: icmp_seq=160, ttl=252, time=583.941984 ms
84 bytes from 10.200.0.1: icmp_seq=161, ttl=252, time=853.806973 ms
84 bytes from 10.200.0.1: icmp_seq=162, ttl=252, time=485.791969 ms
84 bytes from 10.200.0.1: icmp_seq=163, ttl=252, time=755.937958 ms
84 bytes from 10.200.0.1: icmp_seq=164, ttl=252, time=387.768002 ms
84 bytes from 10.200.0.1: icmp_seq=165, ttl=252, time=657.830000 ms
84 bytes from 10.200.0.1: icmp_seq=166, ttl=252, time=289.592981 ms
84 bytes from 10.200.0.1: icmp_seq=167, ttl=252, time=555.747986 ms
84 bytes from 10.200.0.1: icmp_seq=168, ttl=252, time=826.068020 ms
84 bytes from 10.200.0.1: icmp_seq=169, ttl=252, time=457.433987 ms
84 bytes from 10.200.0.1: icmp_seq=170, ttl=252, time=659.357977 ms
84 bytes from 10.200.0.1: icmp_seq=171, ttl=252, time=292.221975 ms
84 bytes from 10.200.0.1: icmp_seq=172, ttl=252, time=561.565971 ms
84 bytes from 10.200.0.1: icmp_seq=173, ttl=252, time=832.812023 ms
84 bytes from 10.200.0.1: icmp_seq=174, ttl=252, time=458.298016 ms
84 bytes from 10.200.0.1: icmp_seq=175, ttl=252, time=732.971954 ms
84 bytes from 10.200.0.1: icmp_seq=176, ttl=252, time=361.752987 ms
84 bytes from 10.200.0.1: icmp_seq=177, ttl=252, time=631.740999 ms
84 bytes from 10.200.0.1: icmp_seq=178, ttl=252, time=263.767004 ms
84 bytes from 10.200.0.1: icmp_seq=179, ttl=252, time=533.651972 ms
84 bytes from 10.200.0.1: icmp_seq=180, ttl=252, time=803.784943 ms
84 bytes from 10.200.0.1: icmp_seq=181, ttl=252, time=433.730984 ms
84 bytes from 10.200.0.1: icmp_seq=182, ttl=252, time=705.822992 ms
84 bytes from 10.200.0.1: icmp_seq=183, ttl=252, time=335.889006 ms
84 bytes from 10.200.0.1: icmp_seq=184, ttl=252, time=607.781982 ms
84 bytes from 10.200.0.1: icmp_seq=185, ttl=252, time=877.666950 ms
84 bytes from 10.200.0.1: icmp_seq=186, ttl=252, time=507.928991 ms
84 bytes from 10.200.0.1: icmp_seq=187, ttl=252, time=780.262995 ms
84 bytes from 10.200.0.1: icmp_seq=188, ttl=252, time=410.839987 ms
84 bytes from 10.200.0.1: icmp_seq=189, ttl=252, time=680.283976 ms
84 bytes from 10.200.0.1: icmp_seq=190, ttl=252, time=326.880002 ms
84 bytes from 10.200.0.1: icmp_seq=191, ttl=252, time=502.359962 ms
84 bytes from 10.200.0.1: icmp_seq=192, ttl=252, time=775.395012 ms
84 bytes from 10.200.0.1: icmp_seq=193, ttl=252, time=408.291960 ms
84 bytes from 10.200.0.1: icmp_seq=194, ttl=252, time=680.260992 ms
84 bytes from 10.200.0.1: icmp_seq=195, ttl=252, time=309.456992 ms
84 bytes from 10.200.0.1: icmp_seq=196, ttl=252, time=581.939030 ms
84 bytes from 10.200.0.1: icmp_seq=197, ttl=252, time=851.758957 ms
84 bytes from 10.200.0.1: icmp_seq=198, ttl=252, time=479.713964 ms
84 bytes from 10.200.0.1: icmp_seq=199, ttl=252, time=749.755001 ms
84 bytes from 10.200.0.1: icmp_seq=200, ttl=252, time=379.848981 ms
200 packets transmitted, 196 packets received
(200, 196)

==> plot/Raw_Data/lte_raw.tex <==
Current Time:24,LTE_Init:2,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:48,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
AAAAAAAAAAAAA
Current Time:69,LTE_Init:2,LTE_Attach:9,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
AAAAAAAAAAAAAAAAAAAAAAAA
Current Time:92,LTE_Init:2,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 0
AAAAAAAAAAAAAAAAAA
Current Time:114,LTE_Init:3,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:143,LTE_Init:2,LTE_Attach:18,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAA
Current Time:166,LTE_Init:2,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAA
Current Time:186,LTE_Init:2,LTE_Attach:8,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAA
Current Time:207,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAA
Current Time:227,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:256,LTE_Init:3,LTE_Attach:16,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAA
Current Time:279,LTE_Init:2,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
AAAAAAAAAAAAAAAA
Current Time:300,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:325,LTE_Init:2,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAA
Current Time:347,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:372,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:405,LTE_Init:2,LTE_Attach:21,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAA
Current Time:426,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
AAAAAAAAAAAAAAAAAC
Current Time:448,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAA
Current Time:469,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:494,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAA
Current Time:515,LTE_Init:2,LTE_Attach:9,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
AAAAAAAAAAAAAA
Current Time:535,LTE_Init:2,LTE_Attach:8,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAA
Current Time:54,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:266,LTE_Init:2,LTE_Attach:50,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:291,LTE_Init:2,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:316,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAA
Current Time:337,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAC
Current Time:358,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:563,LTE_Init:2,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:588,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:614,LTE_Init:3,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:639,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:664,LTE_Init:3,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:53,LTE_Reset:0,LTE_Init:1,LTE_Attach:40,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:103,LTE_Reset:0,LTE_Init:2,LTE_Attach:39,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 0
Current Time:155,LTE_Reset:0,LTE_Init:2,LTE_Attach:40,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:206,LTE_Reset:0,LTE_Init:2,LTE_Attach:40,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:259,LTE_Reset:0,LTE_Init:2,LTE_Attach:41,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:309,LTE_Reset:0,LTE_Init:2,LTE_Attach:38,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
Current Time:361,LTE_Reset:0,LTE_Init:2,LTE_Attach:40,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:411,LTE_Reset:0,LTE_Init:2,LTE_Attach:39,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:462,LTE_Reset:0,LTE_Init:2,LTE_Attach:40,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:488,LTE_Reset:0,LTE_Init:2,LTE_Attach:15,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:568,LTE_Reset:0,LTE_Init:3,LTE_Attach:67,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:617,LTE_Reset:0,LTE_Init:2,LTE_Attach:37,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:667,LTE_Reset:0,LTE_Init:2,LTE_Attach:39,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:720,LTE_Reset:0,LTE_Init:2,LTE_Attach:41,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:769,LTE_Reset:0,LTE_Init:2,LTE_Attach:38,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:796,LTE_Reset:0,LTE_Init:2,LTE_Attach:16,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:875,LTE_Reset:0,LTE_Init:2,LTE_Attach:68,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:988,LTE_Reset:0,LTE_Init:2,LTE_Attach:102,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:1035,LTE_Reset:0,LTE_Init:2,LTE_Attach:35,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:1114,LTE_Reset:0,LTE_Init:2,LTE_Attach:68,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:1165,LTE_Reset:0,LTE_Init:3,LTE_Attach:38,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:1215,LTE_Reset:0,LTE_Init:2,LTE_Attach:38,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:1267,LTE_Reset:0,LTE_Init:2,LTE_Attach:40,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:1292,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:1345,LTE_Reset:0,LTE_Init:2,LTE_Attach:41,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:27,LTE_Reset:0,LTE_Init:4,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:52,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
Current Time:101,LTE_Reset:0,LTE_Init:2,LTE_Attach:37,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
Current Time:123,LTE_Reset:0,LTE_Init:2,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
Current Time:144,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:165,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:202,LTE_Reset:0,LTE_Init:2,LTE_Attach:25,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:226,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:247,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:273,LTE_Reset:0,LTE_Init:2,LTE_Attach:15,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:297,LTE_Reset:0,LTE_Init:3,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:319,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:344,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:364,LTE_Reset:0,LTE_Init:2,LTE_Attach:8,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
Current Time:385,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:411,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:431,LTE_Reset:0,LTE_Init:2,LTE_Attach:8,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
Current Time:451,LTE_Reset:0,LTE_Init:2,LTE_Attach:8,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:472,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:493,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1





Current Time:31,LTE_Reset:8,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 0
Current Time:121,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 0
Current Time:68,LTE_Reset:6,LTE_Init:0,LTE_Attach:16,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:129,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:126,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:192,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:38,LTE_Reset:12,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:56,LTE_Reset:32,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:85,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:116,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:181,LTE_Reset:7,LTE_Init:0,LTE_Attach:46,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:214,LTE_Reset:6,LTE_Init:0,LTE_Attach:15,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 2
Current Time:243,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:273,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:304,LTE_Reset:6,LTE_Init:0,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:336,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:372,LTE_Reset:7,LTE_Init:0,LTE_Attach:17,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:403,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:432,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:463,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:494,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:526,LTE_Reset:6,LTE_Init:0,LTE_Attach:14,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:554,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 0
Current Time:585,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:617,LTE_Reset:7,LTE_Init:0,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:647,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE DeInit: 1
Current Time:677,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE DeInit: 1
Current Time:708,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:739,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:771,LTE_Reset:6,LTE_Init:0,LTE_Attach:14,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1
Current Time:800,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE DeInit: 1




entry 0x400a05bc
AAAAAAAAAAAAAAA
Current Time:30,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAA
Current Time:62,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAA
Current Time:92,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAA
Current Time:124,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAC
Current Time:157,LTE_Reset:6,LTE_Init:0,LTE_Attach:15,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:190,LTE_Reset:6,LTE_Init:0,LTE_Attach:15,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:221,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAC
Current Time:252,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:280,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:312,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:343,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAA
Current Time:373,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAA
Current Time:405,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:434,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:465,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:497,LTE_Reset:6,LTE_Init:0,LTE_Attach:15,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:526,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:558,LTE_Reset:7,LTE_Init:0,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:589,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:619,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:650,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAC
Current Time:682,LTE_Reset:6,LTE_Init:0,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:711,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 0,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:744,LTE_Reset:6,LTE_Init:0,LTE_Attach:15,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:775,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:803,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:834,LTE_Reset:7,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAC
Current Time:866,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:895,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 0,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAA
Current Time:926,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAA
Current Time:957,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAA
Current Time:989,LTE_Reset:6,LTE_Init:0,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:1024,LTE_Reset:6,LTE_Init:0,LTE_Attach:17,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:1054,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:1087,LTE_Reset:6,LTE_Init:0,LTE_Attach:15,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:1116,LTE_Reset:6,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:1146,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAA
Current Time:1178,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:1209,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:1239,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:1269,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:1301,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:1331,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:1361,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:1392,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:1424,LTE_Reset:7,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAA
Current Time:1455,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAA
Current Time:1485,LTE_Reset:6,LTE_Init:0,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAA
Current Time:1515,LTE_Reset:7,LTE_Init:0,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:1546,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:1576,LTE_Reset:6,LTE_Init:0,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0


AAAAAAAAAAAAAAAAAAAAA
Current Time:24,LTE_Reset:0,LTE_Init:1,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:49,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAA
Current Time:70,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAA
Current Time:90,LTE_Reset:0,LTE_Init:2,LTE_Attach:8,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:114,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAA
Current Time:136,LTE_Reset:0,LTE_Init:3,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 0,LTE DeInit: 0
AAAAAAAAAAAAAAC
Current Time:157,LTE_Reset:0,LTE_Init:3,LTE_Attach:8,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:183,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:208,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAA
Current Time:228,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAC
Current Time:249,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:276,LTE_Reset:0,LTE_Init:2,LTE_Attach:15,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:301,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAA
Current Time:325,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 0,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:347,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:379,LTE_Reset:0,LTE_Init:2,LTE_Attach:20,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:402,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:426,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:450,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:474,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAA
Current Time:495,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:521,LTE_Reset:0,LTE_Init:2,LTE_Attach:15,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:546,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:572,LTE_Reset:0,LTE_Init:3,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:597,LTE_Reset:0,LTE_Init:3,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 0,LTE DeInit: 1
AAAAAAAAAAAAAAA
Current Time:618,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:643,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAA
Current Time:663,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAA
Current Time:684,LTE_Reset:0,LTE_Init:2,LTE_Attach:9,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAA
Current Time:706,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:732,LTE_Reset:0,LTE_Init:3,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:757,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 0,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:790,LTE_Reset:0,LTE_Init:2,LTE_Attach:22,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAA
Current Time:812,LTE_Reset:0,LTE_Init:2,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:838,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:863,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:887,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAA
Current Time:910,LTE_Reset:0,LTE_Init:2,LTE_Attach:11,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 2,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:936,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:961,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:985,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAA
Current Time:1006,LTE_Reset:0,LTE_Init:2,LTE_Attach:10,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 0,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAA
Current Time:1029,LTE_Reset:0,LTE_Init:2,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:1054,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:1079,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:1105,LTE_Reset:0,LTE_Init:2,LTE_Attach:14,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAAAA
Current Time:1130,LTE_Reset:0,LTE_Init:2,LTE_Attach:13,LTE_Connect:1,LTE_Disconnect:8,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAA
Current Time:1150,LTE_Reset:0,LTE_Init:2,LTE_Attach:8,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:1174,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 0
AAAAAAAAAAAAAAAAAAAAA
Current Time:1198,LTE_Reset:0,LTE_Init:2,LTE_Attach:11,LTE_Connect:2,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1
AAAAAAAAAAAAAAAAAAAAAAA
Current Time:1222,LTE_Reset:0,LTE_Init:2,LTE_Attach:12,LTE_Connect:1,LTE_Disconnect:7,LTE Detach: 1,LTE DeInit: 1




Socket Send Time
P1SF7,2020-08-20 21:48:15,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF7,2020-08-20 21:48:25,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF7,2020-08-20 21:48:35,InitTime:0,JoinTime:6,sock_time:0,send_Time:179
P1SF7,2020-08-20 21:48:45,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF7,2020-08-20 21:48:55,InitTime:0,JoinTime:6,sock_time:0,send_Time:180
P1SF7,2020-08-20 21:49:05,InitTime:0,JoinTime:6,sock_time:0,send_Time:177
P1SF7,2020-08-20 21:49:15,InitTime:0,JoinTime:6,sock_time:0,send_Time:178
P1SF7,2020-08-20 21:49:25,InitTime:0,JoinTime:6,sock_time:0,send_Time:179
P1SF7,2020-08-20 21:49:35,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF7,2020-08-20 21:49:45,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF12,2020-08-20 21:51:21,InitTime:0,JoinTime:6,sock_time:0,send_Time:175
P1SF12,2020-08-20 21:51:31,InitTime:0,JoinTime:6,sock_time:0,send_Time:177
P1SF12,2020-08-20 21:51:41,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF12,2020-08-20 21:51:51,InitTime:0,JoinTime:6,sock_time:0,send_Time:177
P1SF12,2020-08-20 21:52:01,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF12,2020-08-20 21:52:11,InitTime:0,JoinTime:6,sock_time:0,send_Time:181
P1SF12,2020-08-20 21:52:21,InitTime:0,JoinTime:6,sock_time:0,send_Time:173
P1SF12,2020-08-20 21:52:31,InitTime:0,JoinTime:6,sock_time:0,send_Time:175
P1SF12,2020-08-20 21:52:41,InitTime:0,JoinTime:6,sock_time:0,send_Time:173
P1SF12,2020-08-20 21:52:51,InitTime:0,JoinTime:6,sock_time:0,send_Time:177
P242SF7,2020-08-20 22:04:26,InitTime:0,JoinTime:6,sock_time:0,send_Time:156
P242SF7,2020-08-20 22:04:36,InitTime:0,JoinTime:6,sock_time:0,send_Time:160
P242SF7,2020-08-20 22:04:46,InitTime:0,JoinTime:6,sock_time:0,send_Time:158
P242SF7,2020-08-20 22:04:56,InitTime:0,JoinTime:6,sock_time:0,send_Time:161
P242SF7,2020-08-20 22:05:06,InitTime:0,JoinTime:6,sock_time:0,send_Time:161
P242SF7,2020-08-20 22:05:16,InitTime:0,JoinTime:6,sock_time:0,send_Time:160
P242SF7,2020-08-20 22:05:26,InitTime:0,JoinTime:6,sock_time:0,send_Time:158
P242SF7,2020-08-20 22:05:36,InitTime:0,JoinTime:6,sock_time:0,send_Time:160
P242SF7,2020-08-20 22:05:46,InitTime:0,JoinTime:6,sock_time:0,send_Time:158
P242SF7,2020-08-20 22:05:56,InitTime:0,JoinTime:6,sock_time:0,send_Time:161
P51SF12,2020-08-20 22:16:19,InitTime:0,JoinTime:6,sock_time:0,send_Time:142
P51SF12,2020-08-20 22:16:29,InitTime:0,JoinTime:6,sock_time:0,send_Time:146
P51SF12,2020-08-20 22:16:39,InitTime:0,JoinTime:6,sock_time:0,send_Time:146
P51SF12,2020-08-20 22:16:49,InitTime:0,JoinTime:6,sock_time:0,send_Time:143
P51SF12,2020-08-20 22:16:59,InitTime:0,JoinTime:6,sock_time:0,send_Time:146
P51SF12,2020-08-20 22:17:09,InitTime:0,JoinTime:6,sock_time:0,send_Time:144
P51SF12,2020-08-20 22:17:19,InitTime:0,JoinTime:6,sock_time:0,send_Time:147
P51SF12,2020-08-20 22:17:29,InitTime:0,JoinTime:6,sock_time:0,send_Time:151
P51SF12,2020-08-20 22:17:39,InitTime:0,JoinTime:6,sock_time:0,send_Time:146
P51SF12,2020-08-20 22:17:49,InitTime:0,JoinTime:6,sock_time:0,send_Time:147

==> plot/Raw_Data/sigfox_avg_quality.tex <==
Average LQI 

Run 1

A,2020-08-14 17:47:37,MSize: 1,T:09,RB:2020-08-14 17:47:39 
A,2020-08-14 17:47:46,MSize: 2,T:09,RB:2020-08-14 17:47:48
A,2020-08-14 17:47:55,MSize: 3,T:10,RB:2020-08-14 17:48:00	
A,2020-08-14 17:48:05,MSize: 4,T:10,RB:2020-08-14 17:48:07
A,2020-08-14 17:48:15,MSize: 5,T:10,RB:2020-08-14 17:48:24
A,2020-08-14 17:48:25,MSize: 6,T:11,RB:lost	
A,2020-08-14 17:48:36,MSize: 7,T:10,RB:2020-08-14 17:48:45
A,2020-08-14 17:48:46,MSize: 8,T:11,RB:2020-08-14 17:48:55
A,2020-08-14 17:48:57,MSize: 9,T:11,RB:2020-08-14 17:49:03
A,2020-08-14 17:49:08,MSize: 10,T:12,RB:2020-08-14 17:49:11
A,2020-08-14 17:49:20,MSize: 11,T:11,RB:Lost
A,2020-08-14 17:49:31,MSize: 12,T:12,RB:2020-08-14 17:49:41

Run 2:

A,2020-08-14 21:49:29,MSize:1,Time:9,RB:2020-08-14 21:49:31
A,2020-08-14 21:49:38,MSize:2,Time:9,RB:2020-08-14 21:49:40
A,2020-08-14 21:49:47,MSize:3,Time:10,RB:2020-08-14 21:49:50
A,2020-08-14 21:49:57,MSize:4,Time:10,RB:2020-08-14 21:49:59
A,2020-08-14 21:50:07,MSize:5,Time:10,RB:2020-08-14 21:50:09
A,2020-08-14 21:50:17,MSize:6,Time:11,RB:2020-08-14 21:50:20
A,2020-08-14 21:50:28,MSize:7,Time:10,RB:2020-08-14 21:50:30
A,2020-08-14 21:50:38,MSize:8,Time:11,RB:2020-08-14 21:50:44
A,2020-08-14 21:50:49,MSize:9,Time:11,RB:2020-08-14 21:50:52
A,2020-08-14 21:51:00,MSize:10,Time:12,RB:2020-08-14 21:51:03
A,2020-08-14 21:51:12,MSize:11,Time:11,RB:2020-08-14 21:51:15
A,2020-08-14 21:51:23,MSize:12,Time:12,RB:2020-08-14 21:51:26

Run 3

A,2020-08-14 21:57:10,MSize:1,Time:9,RB:2020-08-14 21:57:11
A,2020-08-14 21:57:19,MSize:2,Time:9,RB:2020-08-14 21:57:20	
A,2020-08-14 21:57:28,MSize:3,Time:10,RB:2020-08-14 21:57:30
A,2020-08-14 21:57:38,MSize:4,Time:9,RB:2020-08-14 21:57:40
A,2020-08-14 21:57:47,MSize:5,Time:11,RB:2020-08-14 21:57:50
A,2020-08-14 21:57:58,MSize:6,Time:11,RB:2020-08-14 21:58:00
A,2020-08-14 21:58:09,MSize:7,Time:10,RB:2020-08-14 21:58:11
A,2020-08-14 21:58:19,MSize:8,Time:11,RB:2020-08-14 21:58:22
A,2020-08-14 21:58:30,MSize:9,Time:11,RB:2020-08-14 21:58:36
A,2020-08-14 21:58:41,MSize:10,Time:12,RB:2020-08-14 21:58:44
A,2020-08-14 21:58:53,MSize:11,Time:11,RB:2020-08-14 21:58:55
A,2020-08-14 21:59:04,MSize:12,Time:12,RB:2020-08-14 21:59:11


Good LQI

G,2020-08-14 18:32:16,MSize: 1,T:9,RB:2020-08-14 18:32:18	
G,2020-08-14 18:32:25,MSize: 2,T:10,RB:2020-08-14 18:32:27
G,2020-08-14 18:32:35,MSize: 3,T:9,RB:2020-08-14 18:32:37
G,2020-08-14 18:32:44,MSize: 4,T:10,RB:2020-08-14 18:32:46
G,2020-08-14 18:32:54,MSize: 5,T:10,RB:2020-08-14 18:32:56
G,2020-08-14 18:33:04,MSize: 6,T:11,RB:2020-08-14 18:33:07
G,2020-08-14 18:33:15,MSize: 7,T:11,RB:2020-08-14 18:33:18
G,2020-08-14 18:33:26,MSize: 8,T:10,RB:2020-08-14 18:33:28
G,2020-08-14 18:33:36,MSize: 9,T:12,RB:2020-08-14 18:33:39
G,2020-08-14 18:33:48,MSize: 10,T:11,RB:2020-08-14 18:33:50
G,2020-08-14 18:33:59,MSize: 11,T:12,RB:2020-08-14 18:34:02
G,2020-08-14 18:34:11,MSize: 12,T:11,RB:2020-08-14 18:34:14

Excellent LQI


E,2020-08-14 19:17:38,MSize: 1,T:9,RB:2020-08-14 19:17:40
E,2020-08-14 19:17:47,MSize: 2,T:9,RB:2020-08-14 19:17:49
E,2020-08-14 19:17:56,MSize: 3,T:10,RB:2020-08-14 19:17:59
G,2020-08-14 19:18:06,MSize: 4,T:10,RB:2020-08-14 19:18:08
E,2020-08-14 19:18:16,MSize: 5,T:10,RB:2020-08-14 19:18:17
E,2020-08-14 19:18:26,MSize: 6,T:11,RB:2020-08-14 19:18:29
E,2020-08-14 19:18:37,MSize: 7,T:10,RB:2020-08-14 19:18:40
E,2020-08-14 19:18:47,MSize: 8,T:11,RB:2020-08-14 19:18:50
G,2020-08-14 19:18:58,MSize: 9,T:11,RB:2020-08-14 19:19:01
G,2020-08-14 19:19:09,MSize: 10,T:12,RB:2020-08-14 19:19:13
E,2020-08-14 19:16:24,MSize: 11,T:12,RB:2020-08-14 19:16:27
E,2020-08-14 19:16:36,MSize: 12,T:11,RB:2020-08-14 19:16:39


G->E
4,9,10

Sigfox socket almost created instantaneously 


One Bit Message

Average

2020-08-20 20:41:39 - 1 bit - 2020-08-20 20:41:41
2020-08-20 20:46:03 - 1 bit - 2020-08-20 20:46:05
2020-08-20 20:50:12 - 1 bit - 2020-08-20 20:50:14	

Good 

2020-08-20 20:43:25 - 1 bit - 	2020-08-20 20:43:26
2020-08-20 20:48:26 - 1 bit -   2020-08-20 20:48:27

==> plot/Raw_Data/wificonnect_raw.tex <==
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit1
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:4,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit1
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:2,Connect:6,Disconnect:0,Dinit0
Init:0,Scan:3,Connect:6,Disconnect:0,Dinit0
